Robust global supply chain reconfiguration under tariff and geopolitical uncertainty

Global supply chains are increasingly exposed to trade policy shocks and physical disruptions arising from common geopolitical events. We develop a robust optimization framework with two decision stages for strategic supply chain reconfiguration. Supplier qualification and transportation arc activation decisions are made before uncertainty is realized, while operational flows adapt afterward. Geopolitical uncertainty is represented through country level shocks that can jointly trigger tariff escalation, policy induced restrictions on cross border capacity, facility disruptions, and physical transportation failures. The resulting min max min problem is reformulated by dualizing the operational recourse problem, yielding a nonconvex mixed integer bilinear adversarial problem solved within a column and constraint generation procedure. Comparison with complete enumeration verifies the implementation on small instances, while experiments on 60 synthetic supply chain networks of varying sizes assess computational performance. The results show that omitting geopolitical transmission channels during strategic design can lead to substantial deterioration in cost and service under full geopolitical stress. Broader protection is achieved primarily through changes in transportation network configuration rather than increased supplier qualification. Robust performance also depends on the severity and composition of geopolitical consequences, with restrictions on cross border capacity exerting a stronger effect than comparable proportional changes in tariff severity over the tested ranges. A geographically grounded case analysis further shows that the value of individual uncertainty channels depends on network structure and geographic exposure.

==> repo.tex <==

We consider the strategic reconfiguration of a global supply chain operating under geopolitical uncertainty in which trade-policy changes and physical disruptions occur simultaneously. The supply chain consists of four echelons, namely suppliers, manufacturing plants, warehouses, and retailers, distributed across multiple countries. Materials flow sequentially from suppliers to manufacturing plants, from manufacturing plants to warehouses, and finally from warehouses to retailers. Prior to the realization of uncertainty, the firm determines the strategic structure of the network by selecting suppliers and activating transportation links. Once geopolitical conditions become known, the firm adaptively determines sourcing, production, and distribution decisions using the surviving network. The objective is to identify a network configuration that minimizes long-term strategic investment together with the worst-case operational cost incurred under all admissible realizations of geopolitical uncertainty.

We consider a multi-channel setting in which trade-policy and physical-network consequences originate from common country-level geopolitical shocks. A geopolitical event affecting a particular country may simultaneously trigger tariff escalation on international trade lanes, supplier shutdowns, manufacturing interruptions, warehouse outages, transportation failures, and border restrictions. Consequently, tariff uncertainty and physical disruptions are not modeled as independent uncertainty sources but rather as correlated manifestations of the same underlying geopolitical event. This modeling philosophy provides a more realistic representation of contemporary global supply chain risk while avoiding unrealistic combinations of uncertainty realizations that may arise when different uncertainty sources are modeled independently.

Figure~\ref{fig:framework} illustrates the conceptual framework of the proposed model. The firm first determines the strategic configuration of the supply chain before uncertainty is realized. Nature subsequently selects the worst admissible geopolitical scenario from a country-aware uncertainty set. Finally, after the uncertainty realization becomes known, the firm adaptively determines operational decisions over the surviving network. This sequence naturally gives rise to a two-stage robust optimization problem with adaptive recourse.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Supply Chain Network}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The global supply chain is represented by a directed network
\[
G=(N,E),
\]
where the node set
\[
N=S\cup P\cup W\cup R
\]
consists of four echelons:

\begin{itemize}
\item suppliers $S$,
\item manufacturing plants $P$,
\item warehouses $W$, and
\item retailers $R$.
\end{itemize}

Material flows only between consecutive echelons. Supplier-to-plant transportation links connect suppliers with manufacturing facilities, plant-to-warehouse links connect manufacturing facilities with distribution centers, and warehouse-to-retailer links satisfy customer demand. Each facility possesses finite processing or storage capacity, while each transportation link has limited throughput.

Facilities are geographically distributed across multiple countries. Consequently, transportation links may either be domestic or international. International links are exposed to tariff uncertainty because shipments crossing national borders may experience changes in customs duties or trade regulations. Both domestic and international transportation links remain susceptible to physical disruption caused by geopolitical events.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Strategic Reconfiguration Decisions.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Before uncertainty is realized, the firm determines the long-term configuration of the supply chain. These strategic decisions are referred to as \emph{here-and-now} decisions because they must be implemented prior to observing future geopolitical conditions.

The first-stage decisions include:

\begin{enumerate}

\item qualification or retention of suppliers,

\item activation of transportation links,

\item allocation of strategic investment budget across supplier diversification and transportation redundancy.

\end{enumerate}

Supplier qualification represents investments associated with supplier certification, contractual agreements, auditing, quality verification, regulatory approval, and information-system integration. Similarly, transportation link activation represents long-term logistics contracts, freight-capacity reservation, customs preparation, or maintenance of backup transportation corridors.

These strategic decisions determine the structure of the network that remains available after uncertainty is realized.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Country-Aware Geopolitical Uncertainty.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Following implementation of the strategic network configuration, nature selects an adverse geopolitical scenario from a predefined uncertainty set. Rather than specifying disruptions independently for every facility and transportation link, the proposed framework assumes that uncertainty originates from country-level geopolitical shocks.

A geopolitical shock affecting a country may simultaneously generate several downstream consequences throughout the supply chain, including

\begin{itemize}

\item tariff escalation on international trade lanes,

\item supplier disruptions,

\item manufacturing interruptions,

\item warehouse disruptions,

\item transportation-link failures,

\item border restrictions and customs delays.

\end{itemize}

This coupling mechanism reflects the observation that geopolitical events generally influence multiple components of a supply chain simultaneously rather than producing isolated failures. Consequently, the proposed uncertainty representation explicitly models the dependence among different uncertainty sources through common country-level drivers.

The uncertainty set additionally incorporates geographical exposure budgets, echelon-specific disruption budgets, tariff budgets, and an aggregate joint uncertainty budget that limits the overall severity of simultaneously occurring adverse events. These budgets provide decision makers with considerable flexibility in calibrating the conservatism of the resulting robust optimization model.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Adaptive Operational Decisions.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Once the geopolitical scenario becomes known, the firm adaptively determines operational decisions over the surviving supply chain network. These decisions are referred to as \emph{wait-and-see} decisions because they are made after uncertainty has been observed.

Operational decisions include

\begin{itemize}

\item supplier allocations,

\item production quantities,

\item transportation flows,

\item warehouse shipments,

\item retailer deliveries,

\item unmet customer demand.

\end{itemize}

Because these decisions are scenario dependent, the firm retains operational flexibility while protecting itself against adverse geopolitical realizations. Adaptive recourse therefore constitutes an essential component of the proposed robust optimization framework.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Research Problem.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The objective of this research is to determine the strategic configuration of a global supply chain that minimizes the total cost of network reconfiguration together with the worst-case operational cost under jointly coupled tariff and disruption uncertainty. The resulting optimization model explicitly balances nominal operating efficiency against long-term resilience by jointly considering supplier diversification, transportation redundancy, tariff exposure, and adaptive operational flexibility.

From a methodological perspective, the proposed framework differs from existing robust supply chain design models in three important respects. First, tariff escalation and physical disruptions are modeled as dependent uncertainty sources arising from common country-level geopolitical shocks. Second, strategic network reconfiguration and adaptive operational planning are integrated within a unified two-stage robust optimization framework. Third, the proposed country-aware uncertainty representation captures realistic geopolitical dependence while preserving computational tractability through budgeted uncertainty sets and decomposition-based solution methods.

The following section introduces the notation and develops the mathematical formulation of the proposed two-stage robust optimization model.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Robust Optimization Model}
\label{sec:model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This section develops the proposed two-stage robust optimization model for strategic global supply chain reconfiguration under jointly coupled tariff and geopolitical disruption uncertainty. We first introduce the notation used throughout the paper before presenting the objective function and operational constraints. The uncertainty set governing geopolitical shocks is developed separately in Section~\ref{sec:uncertainty} because it constitutes one of the principal methodological contributions of this work.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Sets and Indices.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The global supply chain is represented by the directed graph

\[
G=(N,E),
\]

where the node set

\[
N=S\cup P\cup W\cup R
\]

contains four echelons consisting of suppliers, manufacturing plants, warehouses, and retailers.

The principal sets used throughout the formulation are summarized in Table~\ref{tab:sets}.

\begin{table}[ht]
\centering
\caption{Sets and indices.}
\label{tab:sets}
\begin{tabular}{ll}
\hline
Notation & Description\\
\hline
$S$ & Set of suppliers\\
$P$ & Set of manufacturing plants\\
$W$ & Set of warehouses\\
$R$ & Set of retailers\\
$C$ & Set of countries\\
$E^{SP}$ & Supplier--plant transportation links\\
$E^{PW}$ & Plant--warehouse transportation links\\
$E^{WR}$ & Warehouse--retailer transportation links\\
$E$ & Complete transportation network\\
$E^{I}$ & International transportation links\\
$E^{D}$ & Domestic transportation links\\
\hline
\end{tabular}
\end{table}

Each facility is associated with exactly one country. Let

\[
\kappa(i)\in C
\]

denote the country in which facility $i$ is located.

International transportation links are defined as

\[
E^{I}
=
\left\{
(i,j)\in E:
\kappa(i)\neq\kappa(j)
\right\},
\]

while all remaining transportation links are domestic.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Parameters.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The principal model parameters are summarized in Table~\ref{tab:parameters}. These parameters describe supplier capacities, transportation capacities, operating costs, tariff rates, customer demand, and strategic investment costs.

\begin{table}[ht]
\centering
\caption{Model parameters.}
\label{tab:parameters}
\begin{tabular}{ll}
\hline
Parameter & Description\\
\hline
$F_s$ & Supplier qualification cost\\
$K_{ij}$ & Transportation link activation cost\\
$U_s$ & Supplier capacity\\
$U_p$ & Plant capacity\\
$U_w$ & Warehouse capacity\\
$u_{ij}$ & Transportation capacity\\
$D_r$ & Retail demand\\
$c_{ij}$ & Operating cost per unit flow\\
$V_{ij}$ & Customs value per unit shipped\\
$\underline{\tau}_{ij}$ & Baseline tariff rate\\
$\overline{\tau}_{ij}$ & Elevated tariff rate\\
$\pi_r$ & Penalty for unmet demand\\
$B$ & Strategic investment budget\\
$\delta_{ij}$ & Fractional cross-border capacity reduction under a policy-induced trade restriction\\
\hline
\end{tabular}
\end{table}

The tariff increase associated with an international transportation link is

\[
\Delta\tau_{ij}
=
\overline{\tau}_{ij}
-
\underline{\tau}_{ij}.
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Decision Variables.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The proposed framework contains three categories of decision variables.

The first category corresponds to strategic network design decisions made before uncertainty is realized.

For every supplier

\[
s\in S,
\]

define

\[
y_s
=
\begin{cases}
1,
&
\text{if supplier $s$ is selected,}
\\[1ex]
0,
&
\text{otherwise.}
\end{cases}
\]

Similarly, for every transportation link

\[
(i,j)\in E,
\]

define

\[
v_{ij}
=
\begin{cases}
1,
&
\text{if transportation link $(i,j)$ is activated,}
\\[1ex]
0,
&
\text{otherwise.}
\end{cases}
\]

The second category consists of uncertainty variables describing geopolitical realizations.

These variables determine

\begin{itemize}

\item country shocks,

\item tariff escalation,

\item cross-border trade-capacity restrictions,

\item supplier disruptions,

\item plant disruptions,

\item warehouse disruptions,

\item transportation failures.

\end{itemize}

Their mathematical definition is deferred to Section~\ref{sec:uncertainty}, where the proposed country-aware uncertainty set is introduced.

The final category consists of adaptive operational variables representing

\begin{itemize}

\item supplier-to-plant shipments,

\item plant-to-warehouse shipments,

\item warehouse-to-retailer shipments,

\item unmet customer demand.

\end{itemize}

These variables are scenario dependent and are determined after the realization of uncertainty.

The complete mathematical formulation is developed in the following subsections.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multi-Channel Geopolitical Uncertainty Architecture}
\label{sec:uncertainty}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A distinguishing feature of the proposed framework is the explicit representation of geopolitical uncertainty through a country-aware uncertainty set. Unlike conventional robust optimization models that treat tariff escalation, facility disruptions, and transportation failures as independent uncertainty sources, we assume that these events originate from common country-level geopolitical shocks. This modeling philosophy is motivated by the observation that contemporary geopolitical events rarely affect a single component of a supply chain in isolation. Instead, trade disputes, economic sanctions, military conflicts, export restrictions, border closures, and diplomatic tensions typically generate multiple disruptions simultaneously across geographically related facilities and transportation corridors.

For example, an escalation in trade tensions between two countries may immediately increase tariffs on cross-border shipments while simultaneously disrupting supplier operations, restricting manufacturing activities, reducing warehouse throughput, and interrupting international transportation corridors. Likewise, regional military conflicts or economic sanctions often affect all facilities located within the impacted geographical region, producing correlated operational and economic disruptions throughout the supply chain. Modeling these uncertainty sources independently therefore ignores an important structural characteristic of modern geopolitical risk and may result in network configurations that either underestimate systemic exposure or become unnecessarily conservative by allowing unrealistic combinations of simultaneous disruptions.

To capture these interactions, we introduce a country-aware uncertainty representation in which geopolitical shocks occur at the country level and subsequently propagate throughout the supply chain. Rather than directly specifying disruptions for individual facilities or transportation links, nature first selects a subset of countries that experience geopolitical stress. The realization of a country-level shock then determines the admissible tariff escalations, supplier disruptions, manufacturing interruptions, warehouse failures, and transportation-link failures associated with the affected countries. Consequently, dependence among different uncertainty sources arises naturally through their common geographical origin.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Country-Level Geopolitical Shocks.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Let

\[
C
\]

denote the set of countries represented in the supply chain network. Every supplier, manufacturing plant, warehouse, and transportation link is associated with one or more countries through its geographical location.

For each country

\[
k\in C,
\]

define the binary variable

\[
g_k=
\begin{cases}
1, & \text{if country }k\text{ experiences a geopolitical shock},\\
0, & \text{otherwise.}
\end{cases}
\]

A geopolitical shock should be interpreted broadly as any adverse event capable of significantly altering international trade conditions or disrupting supply chain operations. Examples include trade sanctions, military conflicts, export restrictions, border closures, major political instability, widespread labor strikes, or severe regulatory interventions. The framework intentionally remains independent of any specific geopolitical event so that it can be applied across a wide range of practical settings.

Since large-scale geopolitical events rarely affect every country simultaneously, the geographical extent of uncertainty is controlled through the budget constraint

\[
\sum_{k\in C} g_k \leq \Gamma_G,
\]

where the parameter $\Gamma_G$ specifies the maximum number of countries that may simultaneously experience geopolitical shocks.

The geographical budget serves two important purposes. First, it prevents unrealistically conservative scenarios in which every country becomes disrupted simultaneously. Second, it allows decision makers to explicitly calibrate the geographical severity of geopolitical uncertainty according to the planning environment under consideration.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Propagation of Geopolitical Shocks.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The realization of country-level shocks propagates throughout the supply chain by affecting multiple operational components simultaneously. Specifically, a shocked country may generate

\begin{itemize}

\item supplier disruptions,

\item manufacturing interruptions,

\item warehouse disruptions,

\item transportation-link failures,

\item tariff escalation on international trade lanes.

\end{itemize}

Let

\[
a_s,\quad
b_p,\quad
d_w,\quad
z_{ij},\quad
q_{ij},\quad
h_{ij}
\]

denote the binary uncertainty variables associated with supplier disruptions, plant disruptions, warehouse disruptions, transportation failures, tariff escalation, and cross-border trade-capacity restrictions, respectively.

Rather than allowing these uncertainty variables to occur independently, we require them to be consistent with the realization of geopolitical shocks.

For every supplier

\[
s\in S,
\]

located in country $\kappa(s)$,

\[
a_s\leq g_{\kappa(s)}.
\]

Similarly,

\[
b_p\leq g_{\kappa(p)},
\qquad
\forall p\in P,
\]

and

\[
d_w\leq g_{\kappa(w)},
\qquad
\forall w\in W.
\]

These constraints ensure that facilities may only become disrupted when their host country experiences a geopolitical shock. Importantly, the converse is not required; a country-level shock does not necessarily imply that every facility within the affected country fails. Consequently, the proposed formulation allows multiple disruption patterns to emerge from the same geopolitical event.

Transportation links connect facilities located in one or more countries. A transportation corridor therefore becomes vulnerable whenever at least one of its endpoint countries experiences a geopolitical shock. Accordingly,

\[
z_{ij}
\leq
g_{\kappa(i)}
+
g_{\kappa(j)},
\qquad
\forall (i,j)\in E.
\]

Finally, tariff escalation is permitted only for international transportation links whose origin or destination countries experience geopolitical stress. Therefore,

\[
q_{ij}
\leq
g_{\kappa(i)}
+
g_{\kappa(j)},
\qquad
\forall (i,j)\in E^{I}.
\]

For the trade-capacity channel, define $h_{ij}=1$ when international lane $(i,j)$ is subject to a geopolitical restriction that reduces usable cross-border capacity. We impose
\[
h_{ij}\leq g_{\kappa(i)}+g_{\kappa(j)},\qquad \forall(i,j)\in E^{I}.
\]
The variable $h_{ij}$ is distinct from the physical-link failure variable $z_{ij}$: $h_{ij}$ represents policy-induced restrictions such as quotas, sanctions, export controls, border restrictions, or customs limitations, whereas $z_{ij}$ represents physical unavailability of the transportation connection.

These coupling constraints constitute the central modeling mechanism of the proposed framework by explicitly linking geopolitical shocks with downstream trade-policy and physical-network consequences.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Budgeted Uncertainty Structure.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Although geopolitical shocks create dependence among uncertainty sources, decision makers often possess additional information regarding the maximum disruption severity that should be protected against. To incorporate such information without sacrificing computational tractability, the proposed framework combines several budget constraints governing different dimensions of uncertainty.

Facility-disruption budgets limit the maximum number of disrupted suppliers, manufacturing plants, and warehouses,

\[
\sum_{s\in S}a_s\leq\Gamma_S,
\]

\[
\sum_{p\in P}b_p\leq\Gamma_P,
\]

\[
\sum_{w\in W}d_w\leq\Gamma_W.
\]

Similarly, transportation failures are independently controlled for each echelon of the supply chain,

\[
\sum_{(s,p)\in E^{SP}}z_{sp}\leq\Gamma_{SP},
\]

\[
\sum_{(p,w)\in E^{PW}}z_{pw}\leq\Gamma_{PW},
\]

\[
\sum_{(w,r)\in E^{WR}}z_{wr}\leq\Gamma_{WR}.
\]

Tariff escalation is limited through

\[
\sum_{(i,j)\in E^{I}}q_{ij}
\leq
\Gamma_T,
\]

where $\Gamma_T$ specifies the maximum number of international trade lanes experiencing elevated tariff regimes. Cross-border trade-capacity restrictions are controlled through
\[
\sum_{(i,j)\in E^{I}}h_{ij}\leq\Gamma_H,
\]
where $\Gamma_H$ limits the number of international lanes simultaneously exposed to policy-induced capacity restrictions.

Finally, all uncertainty sources are integrated through an aggregate joint uncertainty budget,

\[
\lambda_F
\left(
\sum_{s\in S}a_s
+
\sum_{p\in P}b_p
+
\sum_{w\in W}d_w
+
\sum_{(i,j)\in E}z_{ij}
\right)
+
\lambda_T
\sum_{(i,j)\in E^{I}}q_{ij}
+
\lambda_H
\sum_{(i,j)\in E^{I}}h_{ij}
\leq
\Gamma_J.
\]

The weighting parameters $\lambda_F$, $\lambda_T$, and $\lambda_H$ determine the relative contribution of physical disruptions, tariff escalation, and trade-capacity restrictions toward the overall uncertainty budget. This additional level of control enables decision makers to calibrate the relative severity of operational and economic uncertainty according to the planning environment.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Complete Country-Aware Uncertainty Set.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Collecting the preceding constraints, the proposed country-aware uncertainty set is defined as

\[
\mathcal U
=
\left\{
(a,b,d,z,q,h,g): \text{ all country-coupling and budget constraints above are satisfied}
\right\}.
\]

Unlike conventional uncertainty sets that independently specify disruptions for each facility or transportation link, the proposed formulation explicitly recognizes that geopolitical events generate correlated uncertainty across multiple components of the supply chain. This representation captures realistic dependence among tariffs, supplier failures, manufacturing interruptions, warehouse disruptions, and transportation failures while preserving the computational tractability of budgeted robust optimization. Consequently, the uncertainty set provides a unified and interpretable framework for modeling geopolitical risk in strategic supply chain reconfiguration.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Nested Uncertainty Structures and Relationship to Existing Models}
\label{subsec:nesting}

An important property of the proposed framework is that simpler uncertainty environments arise by deactivating selected propagation channels. Let $\mathcal U^{F}$ denote the full multi-channel uncertainty set.

\begin{proposition}[Nesting of restricted uncertainty environments]
Tariff-only, trade-policy-only, and physical-disruption-only uncertainty environments are restrictions of $\mathcal U^{F}$. Specifically, tariff-only uncertainty is obtained by imposing $a=b=d=z=h=0$; trade-policy uncertainty is obtained by imposing $a=b=d=z=0$, leaving $q$ and $h$ active; and physical-disruption uncertainty is obtained by imposing $q=h=0$, leaving $a,b,d,z$ active. Thus each restricted uncertainty set is contained in the full multi-channel uncertainty set when the corresponding budgets are inherited from $\mathcal U^{F}$.
\end{proposition}

\begin{proof}
Each restricted set is obtained from $\mathcal U^{F}$ by adding equality constraints fixing one or more uncertainty-variable families to zero. Adding constraints cannot enlarge the feasible set, which establishes the nesting relationship.
\end{proof}

This proposition concerns the uncertainty architecture rather than every objective function or first-stage decision structure used in prior studies. It therefore permits a precise comparison with tariff, quota, sanction, and physical-disruption models without claiming that every previously published optimization model is algebraically identical to the present formulation. Models in which geopolitical uncertainty operates only through tariff costs and quantitative trade restrictions correspond to the trade-policy branch of the proposed architecture; the full model additionally permits the same country-level shock to propagate into facilities and transportation connectivity.

\subsection{Two-Stage Robust Formulation}
\label{sec:robust_model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Having established the country-aware uncertainty representation, we now formulate the proposed two-stage robust optimization model. The optimization problem consists of three sequential decision makers. In the first stage, the firm determines the strategic configuration of the supply chain by selecting suppliers and activating transportation links before uncertainty is realized. In the second stage, nature selects the worst admissible realization of country-aware geopolitical uncertainty from the uncertainty set developed in Section~\ref{sec:uncertainty}. Finally, after observing the realized geopolitical scenario, the firm adaptively determines sourcing, production, transportation, and distribution decisions over the surviving network.

The resulting optimization problem therefore possesses the classical
\[
\min\text{--}\max\text{--}\min
\]
structure characteristic of two-stage robust optimization with adaptive recourse.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Strategic Reconfiguration Cost.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Prior to the realization of uncertainty, the firm incurs strategic investment costs associated with supplier qualification and transportation network activation.

Let

\[
y_s=
\begin{cases}
1,&\text{if supplier }s\text{ is qualified},\\
0,&\text{otherwise},
\end{cases}
\]

and

\[
v_{ij}=
\begin{cases}
1,&\text{if transportation link }(i,j)\text{ is activated},\\
0,&\text{otherwise}.
\end{cases}
\]

The total strategic reconfiguration cost is therefore

\begin{equation}
C^{R}(y,v)
=
\sum_{s\in S}F_sy_s
+
\sum_{(i,j)\in E}K_{ij}v_{ij},
\label{eq:reconfiguration_cost}
\end{equation}

where the first term represents supplier qualification costs and the second term represents transportation network activation costs.

If the firm possesses a limited strategic investment budget, the first-stage decisions additionally satisfy

\begin{equation}
\sum_{s\in S}F_sy_s
+
\sum_{(i,j)\in E}K_{ij}v_{ij}
\le B.
\label{eq:budget}
\end{equation}

Equation~\eqref{eq:budget} allows decision makers to explicitly control the amount of capital allocated toward resilience investments.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Once uncertainty is realized, the firm determines adaptive operational decisions over the surviving network.

Let

\[
x_{sp},
\qquad
x_{pw},
\qquad
x_{wr},
\]

denote shipment quantities between consecutive echelons, and let

\[
\ell_r
\]

denote unmet customer demand at retailer $r$.

For a fixed first-stage solution $(y,v)$ and a realized uncertainty scenario

\[
\xi=(a,b,d,z,q,h,g)\in\mathcal U,
\]

the operational recourse problem minimizes the total operating cost

\begin{equation}
Q(y,v,\xi)
=
\min
\left\{
C^{O}(x)
+
C^{T}(x,q)
+
C^{L}(\ell)
\right\},
\label{eq:recourse}
\end{equation}

subject to the operational constraints developed below.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Supplier Capacity Constraints.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A supplier may provide material only if it has been qualified during the first stage and remains operational after uncertainty is realized.

Accordingly,

\begin{equation}
\sum_{p:(s,p)\in E^{SP}}
x_{sp}
\le
U_sy_s(1-a_s),
\qquad
\forall s\in S.
\label{eq:supplier_capacity}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Plant Capacity Constraints.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Manufacturing plants possess finite production capacities that become unavailable whenever the corresponding plant is disrupted.

Thus,

\begin{equation}
\sum_{w:(p,w)\in E^{PW}}
x_{pw}
\le
U_p(1-b_p),
\qquad
\forall p\in P.
\label{eq:plant_capacity}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Warehouse Capacity Constraints.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Warehouse throughput is similarly limited by

\begin{equation}
\sum_{r:(w,r)\in E^{WR}}
x_{wr}
\le
U_w(1-d_w),
\qquad
\forall w\in W.
\label{eq:warehouse_capacity}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Transportation Constraints.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Material may traverse a transportation link only if the link has been activated during the first stage and remains operational after the realization of uncertainty.

Therefore,

\begin{equation}
x_{ij}
\le
u_{ij}v_{ij}(1-z_{ij}),
\qquad
\forall(i,j)\in E.
\label{eq:transport_physical}
\end{equation}

For international links, policy-induced trade restrictions impose the additional capacity bound
\begin{equation}
x_{ij}
\le
u_{ij}v_{ij}\left(1-\delta_{ij}h_{ij}\right),
\qquad
\forall(i,j)\in E^{I}.
\label{eq:transport_trade}
\end{equation}

Constraint~\eqref{eq:transport_physical} captures strategic link activation and physical link failure, whereas Constraint~\eqref{eq:transport_trade} captures partial policy-induced loss of usable cross-border capacity. Thus a physical failure forces flow to zero, while a trade restriction reduces usable capacity by the fraction $\delta_{ij}\in[0,1]$. For domestic arcs, $h_{ij}=0$ and $\delta_{ij}=0$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Flow Conservation.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Flow conservation is enforced at every intermediate facility.

For each manufacturing plant,

\begin{equation}
\sum_{s:(s,p)\in E^{SP}}
x_{sp}
=
\sum_{w:(p,w)\in E^{PW}}
x_{pw},
\qquad
\forall p\in P,
\label{eq:plant_balance}
\end{equation}

while each warehouse satisfies

\begin{equation}
\sum_{p:(p,w)\in E^{PW}}
x_{pw}
=
\sum_{r:(w,r)\in E^{WR}}
x_{wr},
\qquad
\forall w\in W.
\label{eq:warehouse_balance}
\end{equation}

These equations assume unit conversion between consecutive echelons. More general production relationships may easily be incorporated without altering the overall optimization framework.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Demand Satisfaction.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Customer demand is either satisfied through the supply chain or recorded as unmet demand.

Accordingly,

\begin{equation}
\sum_{w:(w,r)\in E^{WR}}
x_{wr}
+
\ell_r
=
D_r,
\qquad
\forall r\in R.
\label{eq:demand}
\end{equation}

The shortage variables ensure relatively complete recourse, thereby guaranteeing feasibility even under severe disruption scenarios.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Operating Cost.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The total operating cost consists of three components.

The ordinary operating cost is

\begin{equation}
C^{O}(x)
=
\sum_{(i,j)\in E}
c_{ij}x_{ij},
\label{eq:operating_cost}
\end{equation}

while tariff payments associated with international transportation are

\begin{equation}
C^{T}(x,q)
=
\sum_{(i,j)\in E^{I}}
\left(
\underline{\tau}_{ij}
+
\Delta\tau_{ij}q_{ij}
\right)
V_{ij}x_{ij}.
\label{eq:tariff_cost}
\end{equation}

Finally, unmet customer demand incurs penalty costs

\begin{equation}
C^{L}(\ell)
=
\sum_{r\in R}
\pi_r\ell_r.
\label{eq:shortage_cost}
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Overall Robust Optimization Model.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Combining the strategic reconfiguration cost with the operational recourse model yields the proposed two-stage robust optimization problem

\begin{equation}
\min_{(y,v)\in\mathcal Y}
\left\{
C^{R}(y,v)
+
\max_{\xi\in\mathcal U}
Q(y,v,\xi)
\right\},
\label{eq:robust_model}
\end{equation}

where $\mathcal Y$ denotes the feasible region of the first-stage strategic decisions and $\mathcal U$ represents the country-aware uncertainty set introduced in Section~\ref{sec:uncertainty}.

Substituting the operational recourse problem into
Equation~\eqref{eq:robust_model} yields the equivalent nested optimization problem

\begin{equation}
\min_{(y,v)\in\mathcal Y}
\;
C^{R}(y,v)
+
\max_{\xi\in\mathcal U}
\;
\min_{(x,\ell)\in\mathcal F(y,v,\xi)}
\left\{
C^{O}(x)
+
C^{T}(x,q)
+
C^{L}(\ell)
\right\},
\label{eq:minmaxmin}
\end{equation}

where
$\mathcal F(y,v,\xi)$
denotes the feasible operational region induced by the first-stage decisions and the realized geopolitical scenario.

Equation~\eqref{eq:minmaxmin} captures the sequential interaction between the firm and nature. The outer minimization determines the strategic network configuration before uncertainty is realized. Nature subsequently selects the most adverse country-aware geopolitical scenario contained within the uncertainty set. Finally, after observing the realized uncertainty, the firm adaptively determines sourcing, production, transportation, and distribution decisions that minimize operational cost over the surviving network.

The resulting formulation constitutes a mixed-integer two-stage robust optimization problem with adaptive recourse. Owing to the embedded max--min structure, directly solving Equation~\eqref{eq:minmaxmin} is computationally challenging. The following section uses strong duality to eliminate the inner recourse minimization for fixed first-stage decisions and develops the adversarial subproblem used within a column-and-constraint generation procedure. The resulting adversarial formulation is a nonconvex mixed-integer bilinear optimization problem that is solved directly by a global nonconvex solver.

%
%
%
%

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Reformulation and Solution Method}
\label{sec:reformulation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The two-stage robust optimization model in Section~\ref{sec:robust_model} has the classical
\[
\min\text{--}\max\text{--}\min
\]
structure. For fixed first-stage decisions, the middle-level problem selects the most adverse admissible geopolitical realization, while the inner problem determines the least-cost operational response. We eliminate the inner minimization by applying strong duality to the operational recourse linear program. This yields a single adversarial maximization problem over the uncertainty variables and the recourse-dual variables.

A central computational feature of this reformulation is that the right-hand sides of several recourse constraints contain products of first-stage constants, binary uncertainty variables, and continuous dual multipliers after dualization. Consequently, the adversarial problem is a mixed-integer bilinear optimization problem. We do not impose a big-$M$ linearization because such a reformulation would require valid finite a priori bounds on the relevant dual variables. Instead, the bilinear adversarial problem is solved directly using a global nonconvex optimization solver. This choice preserves the original bilinear formulation and avoids introducing unverified dual bounds.

\subsection{Recourse Dualization and Bilinear Adversarial Problem}
\label{sec:dualization}

Consider fixed first-stage decisions $(\bar y,\bar v)$ and a fixed uncertainty realization
\[
\bar\xi=(\bar a,\bar b,\bar d,\bar z,\bar q,\bar h,\bar g)\in\mathcal U.
\]
The operational recourse problem is the linear program
\begin{equation}
Q(\bar y,\bar v,\bar\xi)
=
\min_{x,\ell}
\left\{
\sum_{(i,j)\in E} c_{ij}x_{ij}
+
\sum_{(i,j)\in E^I}
\left(\underline{\tau}_{ij}+\Delta\tau_{ij}\bar q_{ij}\right)V_{ij}x_{ij}
+
\sum_{r\in R}\pi_r\ell_r
\right\},
\label{eq:compact_primal}
\end{equation}
subject to Constraints~\eqref{eq:supplier_capacity}--\eqref{eq:demand}, with the uncertainty variables fixed at $\bar\xi$. Because unmet demand is permitted, the recourse problem remains feasible for every admissible scenario, and because all demands and capacities are finite, its optimal value is finite. Strong duality therefore applies.

For the dual derivation, let
\[
\phi_s\ge0,\qquad
\gamma_p\ge0,\qquad
\theta_w\ge0
\]
denote the dual multipliers associated with supplier, plant, and warehouse capacity constraints, respectively. Let
\[
\alpha_{ij}\ge0,\qquad (i,j)\in E,
\]
denote the multiplier associated with the physical transportation-capacity constraint~\eqref{eq:transport_physical}, and let
\[
\beta_{ij}\ge0,\qquad (i,j)\in E^I,
\]
denote the multiplier associated with the policy-induced cross-border capacity constraint~\eqref{eq:transport_trade}. Finally, let $\rho_p$ and $\psi_w$ be free dual variables associated with plant and warehouse flow conservation, and let $\lambda_r$ be the free multiplier associated with retailer demand balance.

For fixed $(\bar y,\bar v)$, merging the recourse dual with nature's maximization gives the adversarial problem
\begin{align}
\max_{\substack{\xi\in\mathcal U,\\
\phi,\gamma,\theta,\alpha,\beta,\rho,\psi,\lambda}}
\quad
&
\sum_{r\in R}D_r\lambda_r
-
\sum_{s\in S}
U_s\bar y_s(1-a_s)\phi_s
-
\sum_{p\in P}
U_p(1-b_p)\gamma_p
\nonumber\\
&
-
\sum_{w\in W}
U_w(1-d_w)\theta_w
-
\sum_{(i,j)\in E}
u_{ij}\bar v_{ij}(1-z_{ij})\alpha_{ij}
\nonumber\\
&
-
\sum_{(i,j)\in E^I}
u_{ij}\bar v_{ij}
\left(1-\delta_{ij}h_{ij}\right)\beta_{ij}.
\label{eq:adversarial_bilinear}
\end{align}

The dual-feasibility constraints depend on the echelon of each transportation link. For supplier--plant links,
\begin{align}
-\phi_s+\rho_p-\alpha_{sp}
&\le c_{sp},
&& (s,p)\in E^{SP}\cap E^D,
\label{eq:dual_sp_domestic}\\
-\phi_s+\rho_p-\alpha_{sp}-\beta_{sp}
&\le
c_{sp}
+
\left(\underline{\tau}_{sp}+\Delta\tau_{sp}q_{sp}\right)V_{sp},
&& (s,p)\in E^{SP}\cap E^I.
\label{eq:dual_sp_international}
\end{align}
For plant--warehouse links,
\begin{align}
-\gamma_p-\rho_p+\psi_w-\alpha_{pw}
&\le c_{pw},
&& (p,w)\in E^{PW}\cap E^D,
\label{eq:dual_pw_domestic}\\
-\gamma_p-\rho_p+\psi_w-\alpha_{pw}-\beta_{pw}
&\le
c_{pw}
+
\left(\underline{\tau}_{pw}+\Delta\tau_{pw}q_{pw}\right)V_{pw},
&& (p,w)\in E^{PW}\cap E^I.
\label{eq:dual_pw_international}
\end{align}
For warehouse--retailer links,
\begin{align}
-\theta_w-\psi_w+\lambda_r-\alpha_{wr}
&\le c_{wr},
&& (w,r)\in E^{WR}\cap E^D,
\label{eq:dual_wr_domestic}\\
-\theta_w-\psi_w+\lambda_r-\alpha_{wr}-\beta_{wr}
&\le
c_{wr}
+
\left(\underline{\tau}_{wr}+\Delta\tau_{wr}q_{wr}\right)V_{wr},
&& (w,r)\in E^{WR}\cap E^I.
\label{eq:dual_wr_international}
\end{align}
The shortage variables imply
\begin{equation}
\lambda_r\le\pi_r,\qquad r\in R.
\label{eq:dual_shortage}
\end{equation}

Equations~\eqref{eq:adversarial_bilinear}--\eqref{eq:dual_shortage}, together with the country-coupling and uncertainty-budget constraints defining $\mathcal U$, form the adversarial subproblem used in the computational implementation.

\paragraph{Bilinear structure and solution strategy.}
The nonlinearities arise from terms such as
\[
a_s\phi_s,\qquad
b_p\gamma_p,\qquad
d_w\theta_w,\qquad
z_{ij}\alpha_{ij},\qquad
h_{ij}\beta_{ij}.
\]
In contrast, tariff uncertainty $q_{ij}$ enters the dual-feasibility constraints linearly through the realized unit transportation cost and therefore does not itself require a binary--continuous product in the present formulation.

A standard exact big-$M$ reformulation of a product between a binary uncertainty variable and a continuous dual variable would require valid finite lower and upper bounds on that dual variable. We do not assume such bounds are available. Accordingly, no big-$M$ or McCormick linearization is imposed on the adversarial problem. Instead, the mixed-integer bilinear formulation is passed directly to Gurobi with its nonconvex global-optimization capability enabled (\texttt{NonConvex=2}). The adversarial problem is solved to global optimality within the prescribed solver tolerances.

This distinction is important for the interpretation of the solution method. Strong duality provides an exact reformulation of the inner recourse problem for each fixed uncertainty realization. The resulting adversarial formulation remains bilinear; its global solution is obtained computationally rather than through an auxiliary bounded-dual MILP reformulation. The complete-enumeration experiments in Section~\ref{sec:computational_evaluation} provide an independent primal-based validation of the resulting CCG implementation on small instances.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Column-and-Constraint Generation}
\label{sec:algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Although strong duality eliminates the inner recourse minimization, directly solving the full robust problem remains computationally challenging for realistically sized supply chain networks. The principal source of computational difficulty is the exponentially large number of admissible geopolitical scenarios contained in the country-aware uncertainty set. Explicit enumeration of every uncertainty realization is therefore computationally impractical even for moderately sized networks.

To overcome this challenge, we develop an exact column-and-constraint generation (CCG) algorithm. Rather than considering all uncertainty realizations simultaneously, the algorithm iteratively generates only those geopolitical scenarios that are necessary for establishing optimality. Beginning with a small subset of representative scenarios, the algorithm alternates between solving a restricted master problem and an adversarial subproblem until no scenario capable of further deteriorating the objective function can be identified.

The proposed decomposition exploits the natural two-stage structure of the robust optimization model. The restricted master problem determines the strategic network configuration while considering only previously generated geopolitical scenarios. The adversarial subproblem subsequently identifies the most damaging geopolitical scenario for the current first-stage solution. Whenever a new worst-case scenario is discovered, it is incorporated into the master problem through additional operational constraints. This iterative process continues until convergence.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Restricted Master Problem.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Suppose that after iteration $k$, the algorithm has generated the scenario set

\[
\widehat{\mathcal U}^{\,k}
=
\left\{
\xi^1,\xi^2,\ldots,\xi^k
\right\}
\subseteq
\mathcal U.
\]

For every scenario

\[
\xi^n\in\widehat{\mathcal U}^{\,k},
\]

a separate operational recourse problem is incorporated into the master formulation.

Let

\[
\theta
\]

denote the worst operational cost among all generated scenarios.

The restricted master problem is

\begin{equation}
\min
\;
C^{R}(y,v)
+
\theta
\label{eq:rmp_obj}
\end{equation}

subject to

\begin{equation}
\theta
\ge
Q(y,v,\xi^n),
\qquad
n=1,\ldots,k,
\label{eq:rmp_theta}
\end{equation}

together with

\begin{itemize}

\item first-stage strategic constraints,

\item investment budget constraints,

\item operational constraints associated with every generated scenario.

\end{itemize}

Since only a subset of all uncertainty realizations is considered, the restricted master problem provides a valid lower bound on the optimal robust objective.

Denote the resulting optimal solution by

\[
(\bar y,\bar v).
\]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Adversarial Subproblem.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

After solving the restricted master problem, the algorithm evaluates the robustness of the candidate first-stage solution by solving an adversarial optimization problem.

Fixing

\[
(\bar y,\bar v),
\]

nature seeks the geopolitical realization producing the largest operational cost,

\begin{equation}
\max_{\xi\in\mathcal U}
Q(\bar y,\bar v,\xi).
\label{eq:adversarial}
\end{equation}

As shown in Section~\ref{sec:reformulation}, this optimization problem is represented as a mixed-integer bilinear model and solved directly using global nonconvex optimization.

Let

\[
\bar\xi
\]

denote the optimal uncertainty realization.

The corresponding objective value

\[
Q(\bar y,\bar v,\bar\xi)
\]

represents the true worst-case operational cost associated with the current strategic network.

Consequently,

\begin{equation}
UB
=
C^{R}(\bar y,\bar v)
+
Q(\bar y,\bar v,\bar\xi)
\end{equation}

provides a valid upper bound on the optimal robust objective.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Scenario Generation.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

If

\[
\bar\xi
\notin
\widehat{\mathcal U}^{\,k},
\]

then the newly identified geopolitical scenario is added to the scenario pool,

\[
\widehat{\mathcal U}^{\,k+1}
=
\widehat{\mathcal U}^{\,k}
\cup
\{\bar\xi\}.
\]

The restricted master problem is subsequently reoptimized using the enlarged scenario set.

If no new worst-case scenario is identified, then the current strategic solution is robustly optimal and the algorithm terminates.

Unlike explicit scenario enumeration, the proposed decomposition generates only uncertainty realizations that actively influence the optimal solution. Consequently, the number of generated scenarios is typically much smaller than the total number of feasible geopolitical realizations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Column-and-Constraint Generation Algorithm.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The complete solution methodology is summarized in Algorithm~\ref{alg:ccg}.

\begin{algorithm}[ht]
\caption{Column-and-Constraint Generation Algorithm}
\label{alg:ccg}

\begin{enumerate}

\item Initialize the scenario set with the nominal geopolitical scenario.

\item Set

\[
LB=-\infty,
\qquad
UB=+\infty.
\]

\item Repeat

\begin{enumerate}

\item Solve the restricted master problem.

\item Obtain the candidate strategic solution
$(\bar y,\bar v)$.

\item Update the lower bound.

\item Solve the adversarial subproblem.

\item Obtain the worst-case geopolitical scenario
$\bar\xi$.

\item Update the upper bound.

\item If
$\bar\xi$
has not been generated previously,
add it to the scenario pool.

\end{enumerate}

\item Until

\[
UB-LB\le\varepsilon.
\]

\item Return the optimal strategic network configuration.

\end{enumerate}

\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Finite Convergence.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The proposed decomposition algorithm possesses finite convergence.

\begin{theorem}

Assume that every uncertainty variable is binary and that the uncertainty set
$\mathcal U$
contains finitely many feasible geopolitical realizations.
Then Algorithm~\ref{alg:ccg} terminates after finitely many iterations and returns an optimal solution to the two-stage robust optimization problem.

\end{theorem}

\begin{proof}

The uncertainty set
$\mathcal U$
contains only finitely many feasible geopolitical scenarios because every uncertainty variable is binary and every uncertainty budget is finite.

At each nonterminating iteration, the adversarial subproblem identifies either

\begin{enumerate}

\item a previously generated scenario, implying that no scenario capable of improving the objective exists, or

\item a new geopolitical scenario not contained in the current scenario pool.

\end{enumerate}

In the latter case, exactly one additional scenario is incorporated into the restricted master problem.

Since no scenario can be generated twice and the total number of feasible scenarios is finite, the algorithm must terminate after finitely many iterations.

At termination, the lower and upper bounds coincide within the prescribed tolerance, implying global optimality of the resulting strategic solution.

\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Computational Complexity.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The computational effort of the proposed decomposition algorithm depends primarily on the number of generated geopolitical scenarios rather than the total cardinality of the uncertainty set. Although the complete uncertainty set grows exponentially with network size, empirical evidence in robust optimization indicates that only a relatively small subset of scenarios typically becomes active at optimality.

Each iteration requires the solution of one mixed-integer restricted master problem and one nonconvex mixed-integer bilinear adversarial problem. Both models remain significantly smaller than the deterministic equivalent obtained through complete scenario enumeration. Consequently, the proposed decomposition avoids explicit enumeration of every admissible geopolitical realization. When each restricted master problem and adversarial subproblem is solved to the prescribed global optimality tolerances, the CCG lower- and upper-bound logic provides a certificate of robust optimality to those tolerances.

The following section presents an extensive computational study designed to evaluate the effectiveness of the proposed methodology and to investigate the managerial implications of explicitly modeling country-aware geopolitical uncertainty.
%
%
%
%
%
%
\section{Computational Study}\label{sec:computational_evaluation}

The computational study evaluates the methodological validity, decision-making value, and computational performance of the proposed country-aware robust supply chain reconfiguration framework. Specifically, the experiments examine whether the proposed column-and-constraint generation (CCG) algorithm correctly solves the robust optimization problem, whether jointly representing tariff escalation and physical disruptions produces more resilient network configurations than simpler benchmark models, and whether the proposed method remains computationally effective as the supply chain network increases in size.

The computational analysis addresses the following three research questions.

\begin{enumerate}
    \item[\textbf{RQ1.}] \textbf{Algorithmic correctness.} Does the proposed CCG algorithm recover the same optimal robust solution as complete enumeration on instances for which all feasible uncertainty scenarios can be explicitly generated?

    \item[\textbf{RQ2.}] \textbf{Value of joint country-aware modeling.} How does the proposed model perform relative to deterministic, tariff-only, trade-policy-only, and disruption-only models when all resulting strategic network configurations are evaluated under the same joint tariff--disruption uncertainty environment?

    \item[\textbf{RQ3.}] \textbf{Computational scalability.} How do solution time, the number of generated scenarios, the number of CCG iterations, and the final optimality gap change as the supply chain network becomes larger?
\end{enumerate}

The experimental design is intentionally focused. Its purpose is not to investigate every possible interaction among the model parameters. Instead, the experiments provide direct evidence concerning the numerical correctness of the solution method, the strategic value of jointly modeling tariff and disruption uncertainty, and the computational scalability of the proposed framework.

\paragraph{Test-Instance Classes.}
\label{subsec:test_instance_classes}

The computational experiments use synthetic four-echelon supply chain networks consisting of suppliers, manufacturing plants, warehouses, and retailers. The facilities are distributed across multiple countries, allowing tariffs, facility disruptions, and transportation failures to be linked through common country-level geopolitical shocks.

Four network-size classes are considered. Their dimensions are summarized in Table~\ref{tab:instance_classes}.

\begin{table}[htbp]
\centering
\caption{Supply chain test-instance classes.}
\label{tab:instance_classes}
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Instance class}
&
\textbf{Suppliers}
&
\textbf{Plants}
&
\textbf{Warehouses}
&
\textbf{Retailers}
&
\textbf{Countries}
\\
\midrule
Small      & 8  & 4  & 6  & 12 & 4  \\
Medium     & 15 & 8  & 12 & 25 & 6  \\
Large      & 25 & 12 & 20 & 40 & 8  \\
Very large & 40 & 20 & 30 & 60 & 10 \\
\bottomrule
\end{tabular}
\end{table}

The small instances are used primarily for algorithmic verification because their uncertainty spaces remain sufficiently limited to permit complete scenario enumeration under reduced uncertainty budgets. The medium instances are used for the benchmark-model comparison and the tariff-budget sensitivity analysis. These networks are sufficiently large to exhibit meaningful supplier-diversification, transportation-redundancy, and geographic-exposure decisions while remaining computationally manageable. The large and very-large instances are used primarily to evaluate computational scalability.

Ten independently generated networks are created for each instance class. Therefore, the complete baseline test bed contains
\[
4 \times 10 = 40
\]
supply chain instances.

The ten instances within each class represent ten distinct supply chain networks. They differ in their facility-country assignments, transportation links, capacities, demands, operating costs, strategic costs, tariff rates, and customs values. These ten instances should not be interpreted as ten geopolitical scenarios. For each generated network, the adversarial subproblem identifies the worst admissible geopolitical scenario from the uncertainty set.

Predetermined random seeds are used to make the test instances reproducible. Seeds $1001,\ldots,1010$ are used for the small instances, $2001,\ldots,2010$ for the medium instances, $3001,\ldots,3010$ for the large instances, and $4001,\ldots,4010$ for the very-large instances.

\paragraph{Generation of Test Instances.}
\label{subsec:test_instance_generation}

The instance-generation procedure is designed to produce heterogeneous, sparse, nominally feasible, and reproducible supply chain networks without making data generation itself a separate methodological contribution. A limited number of transparent distributional assumptions is therefore used.

\paragraph{Facility-Country Assignments.}

Each supplier, plant, warehouse, and retailer is assigned to one of the countries represented in the corresponding instance class. Country assignments are generated randomly, subject to the condition that every country contains at least one supply chain facility.

Let
\[
\kappa(i)\in C
\]
denote the country assigned to facility $i$.

A transportation link $(i,j)$ is classified as international when its endpoints are located in different countries:
\[
E^{I}
=
\left\{
(i,j)\in E:
\kappa(i)\neq \kappa(j)
\right\}.
\]

The remaining transportation links are classified as domestic:
\[
E^{D}=E\setminus E^{I}.
\]

This definition ensures that tariff exposure is determined by actual cross-border movement rather than by the echelon to which a transportation link belongs.

\paragraph{Retailer Demand.}

Total system demand is scaled according to the number of retailers:
\[
TD=750|R|.
\]

This specification maintains approximately the same average demand per retailer across the four network-size classes.

For every retailer $r\in R$, an unnormalized demand weight is generated as
\[
\widetilde{d}_{r}\sim U[0.5,1.5].
\]

The demand assigned to retailer $r$ is then
\[
D_{r}
=
TD
\frac{\widetilde{d}_{r}}
{\sum_{r'\in R}\widetilde{d}_{r'}}.
\]

Consequently,
\[
\sum_{r\in R}D_{r}=TD.
\]

The normalized-weight procedure creates differences in retailer demand while preserving the predetermined level of aggregate demand.

\paragraph{Facility Capacities.}

Aggregate capacity at each supply chain echelon is set equal to $120\%$ of total demand. This level of capacity provides moderate operational flexibility under nominal conditions while ensuring that the network remains vulnerable to concentrated facility and transportation disruptions.

Supplier capacities are generated as
\[
U_{s}
=
1.2TD
\frac{\widetilde{u}_{s}}
{\sum_{s'\in S}\widetilde{u}_{s'}},
\qquad
\widetilde{u}_{s}\sim U[0.5,1.5].
\]

Plant capacities are generated as
\[
U_{p}
=
1.2TD
\frac{\widetilde{u}_{p}}
{\sum_{p'\in P}\widetilde{u}_{p'}},
\qquad
\widetilde{u}_{p}\sim U[0.7,1.3].
\]

Warehouse capacities are generated as
\[
U_{w}
=
1.2TD
\frac{\widetilde{u}_{w}}
{\sum_{w'\in W}\widetilde{u}_{w'}},
\qquad
\widetilde{u}_{w}\sim U[0.7,1.3].
\]

The normalized random weights create heterogeneous facility capacities while ensuring that the aggregate capacity at each echelon remains equal to $1.2TD$.

\paragraph{Transportation-Network Generation.}

Transportation links are generated only between consecutive echelons:
\[
S\rightarrow P,
\qquad
P\rightarrow W,
\qquad
W\rightarrow R.
\]

Each possible supplier-to-plant, plant-to-warehouse, and warehouse-to-retailer link is generated independently using the probabilities
\[
p_{SP}=0.40,
\qquad
p_{PW}=0.45,
\qquad
p_{WR}=0.35,
\]
respectively.

After the initial random generation, the network is repaired when necessary to satisfy the following minimum-connectivity conditions:

\begin{enumerate}
    \item every supplier has at least one outgoing supplier-to-plant link;
    \item every plant has at least one incoming and one outgoing link;
    \item every warehouse has at least one incoming and one outgoing link; and
    \item every retailer has at least two incoming warehouse-to-retailer links whenever the number of warehouses permits.
\end{enumerate}

These conditions prevent trivial network disconnection while retaining a sparse transportation structure.

Transportation capacities are generated using the capacities of the endpoint facilities. For an arc $(i,j)\in E$, let $\deg^{+}(i)$ denote the number of outgoing arcs from node $i$ and let $\deg^{-}(j)$ denote the number of incoming arcs to node $j$. The capacity of arc $(i,j)$ is generated as
\[
u_{ij}
=
\eta_{ij}
\min
\left\{
\frac{U_{i}}{\deg^{+}(i)},
\frac{U_{j}}{\deg^{-}(j)}
\right\},
\]
where
\[
\eta_{ij}\sim U[1.1,1.4].
\]

For a retailer node $r$, the quantity $U_r$ in the preceding expression is replaced by its demand $D_r$.

After generating the network topology and capacities, the nominal operational model is solved with all facilities and transportation links available and with no tariff escalation. An instance is retained only when all retailer demand can be satisfied:
\[
\sum_{r\in R}\ell_r=0.
\]

If the nominal feasibility condition is not satisfied, the transportation network is regenerated using the same base seed and a reproducible attempt index.

\paragraph{Operating Costs.}

Ordinary unit operating costs are generated according to the echelon of the transportation link:
\[
c_{sp}\sim U[6,12],
\qquad (s,p)\in E^{SP},
\]
\[
c_{pw}\sim U[3,7],
\qquad (p,w)\in E^{PW},
\]
and
\[
c_{wr}\sim U[1,4],
\qquad (w,r)\in E^{WR}.
\]

Supplier-to-plant links receive the largest cost range because they represent sourcing and long-distance inbound transportation. Plant-to-warehouse links represent regional distribution and receive an intermediate cost range. Warehouse-to-retailer links represent local or downstream delivery and receive the lowest cost range.

International links receive a $25\%$ cross-border operating-cost premium. Thus, for $(i,j)\in E^{I}$,
\[
c_{ij}^{I}=1.25c_{ij}.
\]

This premium represents additional freight complexity, customs documentation, border processing, and international transportation requirements. Tariff payments are not included in $c_{ij}$ because they are modeled separately in the operational objective.

\paragraph{Tariff Parameters.}

For every international transportation link $(i,j)\in E^{I}$, the baseline tariff rate is generated as
\[
\tau_{ij}^{0}\sim U[0.02,0.08].
\]

The possible tariff increase is generated as
\[
\Delta\tau_{ij}\sim U[0.10,0.30].
\]

The elevated tariff rate is therefore
\[
\overline{\tau}_{ij}
=
\tau_{ij}^{0}
+
\Delta\tau_{ij}.
\]

The customs value per unit shipped is generated as
\[
V_{ij}\sim U[20,40].
\]

For domestic transportation links,
\[
\tau_{ij}^{0}=0,
\qquad
\Delta\tau_{ij}=0,
\qquad
V_{ij}=0.
\]

The tariff-related unit cost incurred on an international link under uncertainty realization $q_{ij}$ is
\[
\left(
\tau_{ij}^{0}
+
\Delta\tau_{ij}q_{ij}
\right)V_{ij}.
\]

Accordingly, the total tariff payment on link $(i,j)$ is
\[
\left(
\tau_{ij}^{0}
+
\Delta\tau_{ij}q_{ij}
\right)V_{ij}x_{ij}.
\]

\paragraph{Strategic Costs.}

Supplier qualification costs are generated as
\[
F_s\sim U[400,800],
\qquad s\in S.
\]

These costs represent supplier auditing, qualification, certification, contractual negotiation, regulatory approval, and information-system integration.

Transportation-link activation costs are generated according to the corresponding network echelon:
\[
K_{sp}\sim U[150,300],
\qquad (s,p)\in E^{SP},
\]
\[
K_{pw}\sim U[100,250],
\qquad (p,w)\in E^{PW},
\]
and
\[
K_{wr}\sim U[50,150],
\qquad (w,r)\in E^{WR}.
\]

International transportation links receive a $20\%$ activation-cost premium:
\[
K_{ij}^{I}=1.20K_{ij},
\qquad (i,j)\in E^{I}.
\]

This premium represents the additional contracting, regulatory, customs, and freight-capacity arrangements required to maintain an international transportation relationship.

\paragraph{Shortage Penalties.}

The unmet-demand penalty is selected to ensure that demand is served whenever doing so is physically and economically feasible. Rather than imposing an arbitrarily large penalty, the value is linked to the maximum cost of delivering one unit through a complete supply chain path.

Let
\[
c_{\max}^{\mathrm{path}}
\]
denote the maximum supplier-to-plant-to-warehouse-to-retailer path cost, including the elevated tariff payment on all international links along that path. The shortage penalty is set as
\[
\pi_r
=
5c_{\max}^{\mathrm{path}},
\qquad r\in R.
\]

This construction makes unmet demand substantially more expensive than feasible delivery while avoiding unnecessarily large coefficients that could create numerical instability.

Table~\ref{tab:parameter_generation} summarizes the principal test-instance generation rules.

\begin{table}[htbp]
\centering
\caption{Summary of test-instance parameter generation.}
\label{tab:parameter_generation}
\small
\begin{tabularx}{\textwidth}{
    >{\raggedright\arraybackslash}p{0.26\textwidth}
    >{\raggedright\arraybackslash}p{0.34\textwidth}
    >{\raggedright\arraybackslash}X}
\toprule
\textbf{Parameter}
&
\textbf{Generation rule}
&
\textbf{Purpose}
\\
\midrule
Total demand
&
$TD=750|R|$
&
Scales aggregate demand with network size.
\\

Retailer weights
&
$\widetilde d_r\sim U[0.5,1.5]$
&
Creates heterogeneous retailer demand.
\\

Supplier capacities
&
Normalized $U[0.5,1.5]$ weights with $20\%$ aggregate slack
&
Creates heterogeneous sourcing capacities.
\\

Plant capacities
&
Normalized $U[0.7,1.3]$ weights with $20\%$ aggregate slack
&
Creates heterogeneous production capacities.
\\

Warehouse capacities
&
Normalized $U[0.7,1.3]$ weights with $20\%$ aggregate slack
&
Creates heterogeneous warehouse capacities.
\\

Supplier--plant arcs
&
Bernoulli probability $0.40$
&
Creates sparse sourcing connectivity.
\\

Plant--warehouse arcs
&
Bernoulli probability $0.45$
&
Creates sparse distribution connectivity.
\\

Warehouse--retailer arcs
&
Bernoulli probability $0.35$
&
Creates sparse downstream connectivity.
\\

Arc-capacity multiplier
&
$\eta_{ij}\sim U[1.1,1.4]$
&
Provides moderate routing flexibility.
\\

Supplier--plant cost
&
$U[6,12]$
&
Represents sourcing and inbound logistics.
\\

Plant--warehouse cost
&
$U[3,7]$
&
Represents regional distribution.
\\

Warehouse--retailer cost
&
$U[1,4]$
&
Represents downstream delivery.
\\

Supplier qualification
&
$F_s\sim U[400,800]$
&
Represents supplier-enablement investment.
\\

Supplier--plant activation
&
$K_{sp}\sim U[150,300]$
&
Represents sourcing-link activation.
\\

Plant--warehouse activation
&
$K_{pw}\sim U[100,250]$
&
Represents distribution-link activation.
\\

Warehouse--retailer activation
&
$K_{wr}\sim U[50,150]$
&
Represents market-link activation.
\\

Baseline tariff
&
$\tau_{ij}^{0}\sim U[0.02,0.08]$
&
Represents nominal tariff exposure.
\\

Tariff increase
&
$\Delta\tau_{ij}\sim U[0.10,0.30]$
&
Represents adverse tariff escalation.
\\

Customs value
&
$V_{ij}\sim U[20,40]$
&
Determines the ad valorem tariff payment.
\\
\bottomrule
\end{tabularx}
\end{table}

\paragraph{Baseline Uncertainty Budgets.}
\label{subsec:baseline_uncertainty_budgets}

The baseline uncertainty budgets are scaled according to the sizes of the corresponding sets. This approach makes uncertainty severity comparable across networks of different sizes.

The country-level geopolitical budget is
\[
\Gamma_G
=
\max
\left\{
1,
\left\lceil0.20|C|\right\rceil
\right\}.
\]

The supplier, plant, and warehouse disruption budgets are
\[
\Gamma_S
=
\max
\left\{
1,
\left\lceil0.10|S|\right\rceil
\right\},
\]
\[
\Gamma_P
=
\max
\left\{
1,
\left\lceil0.10|P|\right\rceil
\right\},
\]
and
\[
\Gamma_W
=
\max
\left\{
1,
\left\lceil0.10|W|\right\rceil
\right\}.
\]

The transportation-link disruption budgets are
\[
\Gamma_{SP}
=
\max
\left\{
1,
\left\lceil0.05|E^{SP}|\right\rceil
\right\},
\]
\[
\Gamma_{PW}
=
\max
\left\{
1,
\left\lceil0.05|E^{PW}|\right\rceil
\right\},
\]
and
\[
\Gamma_{WR}
=
\max
\left\{
1,
\left\lceil0.05|E^{WR}|\right\rceil
\right\}.
\]

The tariff-escalation budget is
\[
\Gamma_T
=
\max
\left\{
1,
\left\lceil0.10|E^{I}|\right\rceil
\right\}.
\]

The trade-capacity budget is
\[
\Gamma_H=\max\left\{1,\left\lceil0.10|E^{I}|\right\rceil\right\}.
\]
The weights in the aggregate joint uncertainty budget are fixed at
\[
\lambda_F=\lambda_T=\lambda_H=1.
\]

The baseline joint uncertainty budget is set equal to
\[
\Gamma_J=3.
\]

These values represent a moderate geopolitical-risk environment. A limited number of countries may experience geopolitical shocks, and only a fraction of the facilities, transportation links, and international trade lanes associated with the affected countries may be disrupted or exposed to tariff escalation.

\paragraph{Experiment 1: Verification of the CCG Algorithm.}
\label{subsec:ccg_verification}

The purpose of the first experiment is to verify that the proposed CCG algorithm correctly solves the two-stage robust optimization problem.

Complete enumeration is computationally possible only when the uncertainty space is sufficiently small. Consequently, this experiment uses the ten small instances together with the reduced uncertainty budgets
\[
\Gamma_G=1,
\]
\[
\Gamma_S=\Gamma_P=\Gamma_W=1,
\]
\[
\Gamma_{SP}=\Gamma_{PW}=\Gamma_{WR}=1,
\]
and
\[
\Gamma_T=\Gamma_H=1.
\]

For each small instance, all feasible country-aware uncertainty scenarios are explicitly generated. A deterministic-equivalent robust model is constructed by including one copy of the operational recourse problem for every feasible uncertainty scenario.

The same supply chain instance is then solved using the proposed CCG algorithm. The objective values obtained by complete enumeration and CCG are compared using
\[
\operatorname{Gap}_{i}
=
\frac{
\left|
Z_{i}^{\mathrm{CCG}}
-
Z_{i}^{\mathrm{ENUM}}
\right|
}{
\max
\left\{
1,
\left|
Z_{i}^{\mathrm{ENUM}}
\right|
\right\}
},
\]
where $Z_i^{\mathrm{CCG}}$ is the optimal objective value obtained using CCG and $Z_i^{\mathrm{ENUM}}$ is the optimal objective value obtained using complete enumeration.

The two methods are considered numerically equivalent when
\[
\operatorname{Gap}_{i}\le 10^{-4}.
\]

For every small instance, the following quantities are recorded:

\begin{itemize}
    \item total number of feasible uncertainty scenarios;
    \item objective value obtained through complete enumeration;
    \item objective value obtained through CCG;
    \item relative objective difference;
    \item complete-enumeration runtime;
    \item CCG runtime;
    \item number of CCG iterations; and
    \item number of scenarios generated by CCG.
\end{itemize}

The verification results are reported using Table~\ref{tab:verification_results}.

\begin{table}[htbp]
\centering
\caption{Verification of the CCG algorithm against complete enumeration.}
\label{tab:verification_results}
\scriptsize
\begin{tabularx}{\textwidth}{
    l
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X}
\toprule
\textbf{Instance}
&
\textbf{Feasible scenarios}
&
\textbf{Enumeration objective}
&
\textbf{CCG objective}
&
\textbf{Relative gap}
&
\textbf{Enumeration time}
&
\textbf{CCG time}
&
\textbf{Generated scenarios}
\\
\midrule
Small-1  & -- & -- & -- & -- & -- & -- & -- \\
Small-2  & -- & -- & -- & -- & -- & -- & -- \\
Small-3  & -- & -- & -- & -- & -- & -- & -- \\
Small-4  & -- & -- & -- & -- & -- & -- & -- \\
Small-5  & -- & -- & -- & -- & -- & -- & -- \\
Small-6  & -- & -- & -- & -- & -- & -- & -- \\
Small-7  & -- & -- & -- & -- & -- & -- & -- \\
Small-8  & -- & -- & -- & -- & -- & -- & -- \\
Small-9  & -- & -- & -- & -- & -- & -- & -- \\
Small-10 & -- & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabularx}
\end{table}

This experiment serves two purposes. First, it independently verifies the numerical correctness of the recourse dualization, the globally solved bilinear adversarial subproblem, and the CCG implementation. The enumeration benchmark is constructed directly from primal recourse copies and therefore does not rely on the adversarial dual formulation. Second, the experiment determines whether CCG can establish robust optimality using only a small subset of the complete uncertainty space.

The proportion of feasible uncertainty scenarios generated by CCG is measured using the scenario-retention ratio
\[
SR_i
=
100
\frac{
N_i^{\mathrm{CCG}}
}{
N_i^{\mathrm{ENUM}}
},
\]
where $N_i^{\mathrm{CCG}}$ is the number of scenarios generated by CCG and $N_i^{\mathrm{ENUM}}$ is the total number of feasible uncertainty scenarios.

A small value of $SR_i$ indicates that only a limited portion of the complete uncertainty space is necessary to establish robust optimality.

\paragraph{Experiment 2: Value of Joint Country-Aware Modeling.}
\label{subsec:joint_model_value}

The second experiment evaluates the decision-making value of jointly modeling tariff escalation and physical disruptions through common country-level geopolitical shocks.

Five models are compared.

\paragraph{Deterministic Model.}

The deterministic model ignores geopolitical uncertainty. All uncertainty variables are fixed at zero:
\[
g=a=b=d=z=q=h=0.
\]

The resulting model selects suppliers and activates transportation links using nominal operating conditions.

\paragraph{Tariff-Only Robust Model.}

The tariff-only model considers country shocks and tariff escalation but assumes that all facilities and transportation links remain physically operational:
\[
a=b=d=z=h=0.
\]

The variables $g$ and $q$ remain active, subject to the country and tariff budgets.

\paragraph{Trade-Policy Robust Model.}

The trade-policy model retains country shocks, tariff escalation, and cross-border capacity restrictions while deactivating physical disruptions:
\[a=b=d=z=0.\]
The variables $g$, $q$, and $h$ remain active. This benchmark represents the class of models in which geopolitical uncertainty propagates through trade costs and trade quantities but not through physical facility or transportation failures.

\paragraph{Disruption-Only Robust Model.}

The disruption-only model considers country shocks, facility disruptions, and transportation-link failures but assumes stable tariffs:
\[
q=h=0.
\]

The variables $g$, $a$, $b$, $d$, and $z$ remain active.

\paragraph{Proposed Joint Country-Aware Model.}

The proposed model simultaneously considers
\[
g,\ a,\ b,\ d,\ z,\ q,\ \text{and }h,
\]
together with all country-level propagation constraints, disruption budgets, tariff budgets, and the aggregate joint uncertainty budget.

The five models are solved on the same ten medium instances. Using the same instances creates a paired experimental design and ensures that observed differences arise from the modeling assumptions rather than from random changes in network topology or parameter values.

For every model and every instance, the following quantities are recorded:

\begin{itemize}
    \item total objective value;
    \item supplier-qualification cost;
    \item transportation-link activation cost;
    \item total strategic cost;
    \item worst-case operating cost;
    \item worst-case tariff payment;
    \item worst-case unmet demand;
    \item worst-case service level;
    \item number of qualified suppliers;
    \item number of activated transportation links;
    \item number of countries represented by the selected suppliers; and
    \item CCG solution time and number of iterations, where applicable.
\end{itemize}

Worst-case service level is calculated as
\[
SL
=
1-
\frac{
\sum_{r\in R}\ell_r
}{
\sum_{r\in R}D_r
}.
\]

A critical feature of the comparison is the common reevaluation procedure. The first-stage strategic network configuration obtained from each benchmark model is fixed and reevaluated using the full uncertainty set of the proposed joint country-aware model.

Let
\[
(y^m,v^m)
\]
denote the strategic solution obtained from model $m$. Its worst-case operating cost under the common joint uncertainty set is
\[
WC_m^{J}
=
\max_{\xi\in\mathcal{U}^{J}}
Q(y^m,v^m,\xi),
\]
where $\mathcal{U}^{J}$ denotes the uncertainty set of the proposed joint country-aware model.

The common reevaluation is required because the deterministic, tariff-only, trade-policy-only, and disruption-only models are optimized under weaker uncertainty environments. Their original objective values therefore do not provide a fair comparison of resilience under jointly occurring tariff escalation and physical disruptions.

The percentage improvement of the proposed joint model over benchmark model $m$ is defined as
\[
\operatorname{Improvement}_{m}
=
100
\frac{
WC_m^{J}
-
WC_J^{J}
}{
WC_m^{J}
}.
\]

Similarly, the reduction in worst-case unmet demand is calculated as
\[
\operatorname{ShortageReduction}_{m}
=
100
\frac{
L_m^{J}
-
L_J^{J}
}{
\max\{1,L_m^{J}\}
},
\]
where $L_m^{J}$ is the worst-case unmet demand associated with the strategic solution of model $m$ under the common joint uncertainty set.

The benchmark comparison is summarized using Table~\ref{tab:model_comparison}.

\begin{table}[htbp]
\centering
\caption{Comparison of strategic solutions under common joint-uncertainty evaluation.}
\label{tab:model_comparison}
\scriptsize
\begin{tabularx}{\textwidth}{
    >{\raggedright\arraybackslash}p{0.18\textwidth}
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X}
\toprule
\textbf{Model}
&
\textbf{Strategic cost}
&
\textbf{Joint operating cost}
&
\textbf{Unmet demand}
&
\textbf{Service level}
&
\textbf{Suppliers selected}
&
\textbf{Links activated}
\\
\midrule
Deterministic       & -- & -- & -- & -- & -- & -- \\
Tariff only         & -- & -- & -- & -- & -- & -- \\
Trade policy        & -- & -- & -- & -- & -- & -- \\
Disruption only     & -- & -- & -- & -- & -- & -- \\
Joint country-aware & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabularx}
\end{table}

The reported entries correspond to the mean across the ten medium instances, with sample standard deviations shown in parentheses.

The experiment is intended to identify the resilience premium associated with joint country-aware protection. The deterministic and single-uncertainty models may require lower initial strategic investment, but their network configurations may perform poorly when tariff escalation and physical disruptions occur simultaneously. The proposed joint model may qualify additional suppliers or activate additional transportation links, but these investments are expected to reduce worst-case operating cost and unmet demand under coupled geopolitical events.

\paragraph{Tariff-Budget Sensitivity Analysis.}
\label{subsec:tariff_budget_sensitivity}

A focused sensitivity analysis examines how increasing tariff uncertainty affects the optimal strategic network configuration and worst-case operational performance.

The analysis uses the same ten medium instances employed in Experiment~2. Facility-country assignments, network topology, demands, capacities, operating costs, strategic costs, physical-disruption budgets, and all other parameters remain fixed. Only the tariff-escalation budget is changed.

The tariff budget is varied over
\[
\Gamma_T
\in
\left\{
0,\,
\left\lceil0.05|E^{I}|\right\rceil,\,
\left\lceil0.10|E^{I}|\right\rceil,\,
\left\lceil0.20|E^{I}|\right\rceil
\right\}.
\]

These four values represent no tariff escalation, low tariff uncertainty, moderate tariff uncertainty, and high tariff uncertainty, respectively.

For each tariff-budget level, the proposed joint country-aware model is resolved. The following quantities are recorded:

\begin{itemize}
    \item total strategic cost;
    \item supplier-qualification cost;
    \item transportation-link activation cost;
    \item worst-case operating cost;
    \item worst-case tariff payment;
    \item worst-case unmet demand;
    \item number of qualified suppliers;
    \item number of activated international links; and
    \item number of countries represented in the selected supplier portfolio.
\end{itemize}

The results are summarized using Table~\ref{tab:tariff_sensitivity}.

\begin{table}[htbp]
\centering
\caption{Sensitivity of the optimal solution to the tariff-escalation budget.}
\label{tab:tariff_sensitivity}
\small
\begin{tabularx}{\textwidth}{
    >{\centering\arraybackslash}p{0.18\textwidth}
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X}
\toprule
\textbf{Tariff budget}
&
\textbf{Strategic cost}
&
\textbf{Operating cost}
&
\textbf{Tariff payment}
&
\textbf{Unmet demand}
&
\textbf{Suppliers selected}
\\
\midrule
$0$                         & -- & -- & -- & -- & -- \\
$\lceil0.05|E^{I}|\rceil$   & -- & -- & -- & -- & -- \\
$\lceil0.10|E^{I}|\rceil$   & -- & -- & -- & -- & -- \\
$\lceil0.20|E^{I}|\rceil$   & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabularx}
\end{table}

The experiment determines whether increasing tariff exposure encourages the firm to qualify additional or more geographically diversified suppliers, activate alternative transportation corridors, reduce reliance on a small number of international lanes, or increase strategic investment to protect worst-case service performance.

The marginal effect of increasing the tariff budget from level $h-1$ to level $h$ is measured using
\[
\Delta Z_h
=
Z(\Gamma_T^h)
-
Z(\Gamma_T^{h-1}),
\]
where $Z(\Gamma_T^h)$ denotes the optimal robust objective under tariff-budget level $\Gamma_T^h$.

The corresponding change in worst-case unmet demand is
\[
\Delta L_h
=
L(\Gamma_T^h)
-
L(\Gamma_T^{h-1}).
\]

These quantities indicate whether the effect of tariff uncertainty increases gradually or whether threshold effects arise at particular tariff-budget levels.

\paragraph{Experiment 3: Computational Scalability.}
\label{subsec:computational_scalability}

The third experiment evaluates the computational scalability of the proposed CCG algorithm across the four network-size classes.

The proposed joint country-aware model is solved for ten instances from each class using the baseline uncertainty budgets. The scalability experiment therefore contains 40 optimization runs.

For every run, the following computational quantities are recorded:

\begin{itemize}
    \item total solution time;
    \item total restricted-master-problem solution time;
    \item total adversarial-subproblem solution time;
    \item number of CCG iterations;
    \item number of unique geopolitical scenarios generated;
    \item final lower bound;
    \item final upper bound;
    \item final relative CCG gap;
    \item final solver MIP gap; and
    \item final solution status.
\end{itemize}

The relative CCG gap is calculated as
\[
\operatorname{CCGGap}
=
\frac{
UB-LB
}{
\max\{1,|UB|\}
}.
\]

An instance is considered solved to the prescribed robust optimality tolerance when
\[
\operatorname{CCGGap}
\le 10^{-4}.
\]

The scalability results are reported using Table~\ref{tab:scalability_results}.

\begin{table}[htbp]
\centering
\caption{Computational scalability of the proposed CCG algorithm.}
\label{tab:scalability_results}
\scriptsize
\begin{tabularx}{\textwidth}{
    >{\raggedright\arraybackslash}p{0.14\textwidth}
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X
    >{\centering\arraybackslash}X}
\toprule
\textbf{Class}
&
\textbf{Solved instances}
&
\textbf{Runtime}
&
\textbf{Master time}
&
\textbf{Subproblem time}
&
\textbf{Iterations}
&
\textbf{Final gap}
\\
\midrule
Small      & -- & -- & -- & -- & -- & -- \\
Medium     & -- & -- & -- & -- & -- & -- \\
Large      & -- & -- & -- & -- & -- & -- \\
Very large & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabularx}
\end{table}

For instances solved within the time limit, runtime, iteration count, and scenario count are reported using the mean and sample standard deviation. For instances that reach the time limit, the incumbent upper bound, lower bound, and final relative gap are reported. Instances reaching the time limit are not classified as optimally solved.

The number of generated scenarios is an important indicator of computational scalability. Although the complete uncertainty space grows rapidly with the number of countries, facilities, transportation links, and tariff-exposed lanes, the CCG method generates only scenarios that affect the current candidate network configuration. The practical effectiveness of the algorithm therefore depends on whether the number of generated scenarios remains small relative to the complete uncertainty space.

The experiment examines the relationship among
\[
\text{network size},
\qquad
\text{CCG iterations},
\qquad
\text{generated scenarios},
\qquad
\text{and solution time}.
\]

\paragraph{Replications and Statistical Reporting.}
\label{subsec:replications_reporting}

For each reported quantity $x$, the sample mean over the ten instances in a class is
\[
\overline{x}
=
\frac{1}{10}
\sum_{i=1}^{10}x_i.
\]

The corresponding sample standard deviation is
\[
s_x
=
\sqrt{
\frac{1}{9}
\sum_{i=1}^{10}
\left(
x_i-\overline{x}
\right)^2
}.
\]

Numerical results are reported in the form
\[
\text{mean}\;(\text{standard deviation}).
\]

For example,
\[
142.6\;(18.4)
\]
represents a sample mean of $142.6$ and a sample standard deviation of $18.4$.

Because all benchmark models are solved on the same ten medium instances, the comparisons are paired. For benchmark model $m$, define the instance-level paired difference
\[
\Delta_i^m
=
WC_{i,m}^{J}
-
WC_{i,J}^{J}.
\]

The average paired improvement is
\[
\overline{\Delta}^{m}
=
\frac{1}{10}
\sum_{i=1}^{10}\Delta_i^m.
\]

A positive value indicates that the proposed joint country-aware model achieves a lower worst-case operating cost than benchmark model $m$ under the common joint uncertainty evaluation.

In addition to raw unmet demand, the shortage percentage is calculated as
\[
\operatorname{ShortagePercentage}
=
100
\frac{
\sum_{r\in R}\ell_r
}{
TD
}.
\]

This measure facilitates comparisons across instance classes having different levels of total demand.

The normalized total cost is calculated as
\[
\operatorname{CostPerUnit}
=
\frac{
\text{total cost}
}{
TD
}.
\]

\paragraph{Solver and Implementation Settings.}
\label{subsec:solver_implementation}

All optimization models are implemented in Python and solved using Gurobi Optimizer. The solver and algorithmic parameters used throughout the computational study are summarized in Table~\ref{tab:solver_settings}.

\begin{table}[htbp]
\centering
\caption{Solver and algorithmic settings.}
\label{tab:solver_settings}
\small
\begin{tabular}{lc}
\toprule
\textbf{Parameter} & \textbf{Value} \\
\midrule
MIPGap             & $10^{-6}$ \\
FeasibilityTol     & $10^{-7}$ \\
IntFeasTol         & $10^{-7}$ \\
OptimalityTol      & $10^{-7}$ \\
Threads            & $1$ \\
NonConvex          & $2$ (adversarial subproblem) \\
Presolve           & Automatic \\
Cuts               & Automatic \\
NumericFocus       & $2$ \\
CCG tolerance      & $10^{-5}$ \\
\bottomrule
\end{tabular}
\end{table}

A single computational thread is used to reduce variation caused by parallel execution and to improve the comparability of solution times across instances.

The CCG algorithm terminates when
\[
\frac{
UB-LB
}{
\max\{1,|UB|\}
}
\le 10^{-5}.
\]

At each iteration, the restricted master problem provides a valid lower bound on the robust objective. The adversarial subproblem identifies the most damaging uncertainty realization for the current first-stage solution and provides a corresponding upper bound. A newly identified geopolitical scenario is added to the restricted master problem only when it has not appeared in a previous iteration.

For every optimization run, the implementation records the objective value, strategic decisions, generated uncertainty scenarios, lower and upper bounds, runtime by algorithmic component, number of iterations, final optimality gap, and final solution status.

\paragraph{Summary of the Experimental Design.}
\label{subsec:experimental_design_summary}

The complete computational evaluation consists of three principal experiments.

\begin{enumerate}
    \item \textbf{Algorithm verification.} The ten small instances are solved using both complete uncertainty-scenario enumeration and the proposed CCG algorithm.

    \item \textbf{Model comparison.} The deterministic, tariff-only, trade-policy-only, disruption-only, and proposed full multi-channel models are solved on the same ten medium instances. Their strategic solutions are subsequently reevaluated under a common joint tariff--disruption uncertainty set.

    \item \textbf{Computational scalability.} The proposed CCG algorithm is applied to ten instances from each of the four network-size classes.
\end{enumerate}

In addition, one focused tariff-budget sensitivity analysis is conducted using the ten medium instances.

Experiment~1 establishes the numerical correctness of the proposed solution methodology. Experiment~2 quantifies the value of jointly modeling tariff escalation and physical disruptions through country-level geopolitical coupling. Experiment~3 evaluates the computational scalability of the CCG algorithm. The tariff-budget sensitivity analysis provides a focused managerial assessment of how increasing trade-policy uncertainty affects strategic supply chain reconfiguration decisions.
\paragraph{Results and managerial insights.}\label{sec:results}
The numerical findings will be reported in four parts: algorithmic verification, comparison of restricted and full multi-channel uncertainty models under common stress testing, sensitivity to trade-policy uncertainty, and computational scalability. The managerial analysis will focus on when supplier diversification, transportation redundancy, and geographic diversification become valuable as geopolitical exposure propagates across multiple channels.

% TODO: Insert validated computational results and managerial interpretation.

\section{Conclusions}\label{sec:conclusion}
This paper develops a country-aware robust optimization framework for strategic global supply chain reconfiguration under multi-channel geopolitical uncertainty. The framework allows common country-level shocks to propagate through tariff costs, cross-border trade capacity, facility availability, and transportation connectivity. It integrates strategic supplier and transportation decisions with adaptive operational recourse and uses column-and-constraint generation to avoid explicit enumeration of the complete uncertainty space.

The final version of this section will summarize the principal computational findings, managerial implications, and limitations after the numerical study is completed. Natural extensions include richer multi-product structures, partial rather than binary capacity losses, endogenous recovery decisions, and data-driven calibration of geopolitical dependence and uncertainty budgets.

